Schottky groups cannot act on $\mathbb{P}^{2n}_{\mathbb{C}}$ as subgroups of $PSL(2n+1,\Bbb{C})$

In this paper we look at a special type of discrete subgroups of $PSL_{n+1}(\Bbb{C})$ called Schottky groups. We develop some basic properties of these groups and their limit set when $n > 1$, and we prove that Schottky groups only occur in odd dimensions, {\it i.e.}, they cannot be realized as subgroups of $PSL_{2n+1}(\Bbb{C})$.

==> TeX.tex <==

\textbf{E} & \\
 & \\
 & \\



Espacio Normado & \pageref{}\\
Espacio Vectorial & \pageref{}\\
Espacio Tangente & \pageref{}\\
Exp & \pageref{}\\
 & \\
\textbf{F} & \\
 & \\
 & \\
Familia Equicontinua & \pageref{}\\
Familia Normal & \pageref{}\\
Flujo & \pageref{}\\
Fubini & \pageref{}\\
Funcion de Borel & \pageref{ref:bor}\\
 & \\
\textbf{G} & \\
 & \\
 & \\
Gr\"otzch & \pageref{}\\
 & \\
\textbf{H} & \\
 & \\ 
 & \\
Homotecias Complejas & \pageref{}\\
 & \\
\textbf{I} & \\
 & \\
 & \\
Integrable & \pageref{}\\
 & \\
\textbf{J} & \\
 & \\
 & \\
Jacobiano & \pageref{}\\
 & \\
\textbf {K} & \\
 & \\
 & \\
Kriloff & \pageref{}\\
\textbf{L} & \\
 & \\
 & \\
$L^P$ & \pageref{}\\
$L^{\infty}$ & \pageref{}\\
L\'{\i}mite de q.c. & \pageref{}\\
Ln & \pageref{}\\
Longitud Extremal & \pageref{}\\
Lusin & \pageref{}\\


==> arrsy.tex <==
<!DOCTYPE rdf:RDF SYSTEM "../tpm.dtd">
<rdf:RDF xmlns:rdf="http://www.w3.org/1999/02/22-rdf-syntax-ns#" xmlns:TPM="http://texlive.dante.de/">
  <rdf:Description about="http://texlive.dante.de/texlive/package/kuvio.zip">
    <TPM:Name>kuvio</TPM:Name>
    <TPM:Type>package</TPM:Type>
    <TPM:Date>2003/08/22 17:03:15</TPM:Date>
    <TPM:Version></TPM:Version>
    <TPM:Creator>rahtz</TPM:Creator>
    <TPM:Title>Drawing macros and fonts for diagrams.</TPM:Title>
    <TPM:Size>2208086</TPM:Size>
    <TPM:Description></TPM:Description>
    <TPM:Build>
      <TPM:RunPatterns>
texmf/fonts/source/public/kuvio/*
texmf/fonts/tfm/public/kuvio/*
texmf/tex/latex/kuvio/*
texmf/tpm/package/kuvio.tpm
      </TPM:RunPatterns>
      <TPM:DocPatterns>
texmf/doc/latex/kuvio/*
texmf/doc/latex/kuvio/eps/*
      </TPM:DocPatterns>
      <TPM:SourcePatterns>
texmf/source/latex/kuvio/*
texmf/source/latex/kuvio/arrsy/*
texmf/source/latex/kuvio/doc-src/*
texmf/source/latex/kuvio/doc-src/eg/*
texmf/source/latex/kuvio/doc-src/eps/*
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/*
texmf/source/latex/kuvio/doc-src/macros/carrot/misc/*
texmf/source/latex/kuvio/doc-src/macros/carrot/sfss/*
texmf/source/latex/kuvio/doc-src/macros/carrot/sfss/fs/*
texmf/source/latex/kuvio/doc-src/macros/misc/*
texmf/source/latex/kuvio/doc-src/tdwk/*
      </TPM:SourcePatterns>
    </TPM:Build>
    <TPM:RunFiles size="168451">
texmf/fonts/source/public/kuvio/arrsy.mf
texmf/fonts/source/public/kuvio/arrsy10.mf
texmf/fonts/source/public/kuvio/arrsym.mf
texmf/fonts/tfm/public/kuvio/arrsy10.tfm
texmf/tex/latex/kuvio/arrsy.sty
texmf/tex/latex/kuvio/arrsy.tex
texmf/tex/latex/kuvio/kuvio.sty
texmf/tex/latex/kuvio/kuvio.tex
texmf/tpm/package/kuvio.tpm
    </TPM:RunFiles>
    <TPM:DocFiles size="1209147">
texmf/doc/latex/kuvio/README
texmf/doc/latex/kuvio/eps/face.eps
texmf/doc/latex/kuvio/eps/harebra.eps
texmf/doc/latex/kuvio/eps/plot.eps
texmf/doc/latex/kuvio/examples.pdf
texmf/doc/latex/kuvio/symbols.tex
texmf/doc/latex/kuvio/tdwk.dvi
    </TPM:DocFiles>
    <TPM:SourceFiles size="830488">
texmf/source/latex/kuvio/COPYRIGHT
texmf/source/latex/kuvio/README
texmf/source/latex/kuvio/README2
texmf/source/latex/kuvio/arrsy/Makefile-dist
texmf/source/latex/kuvio/arrsy/README
texmf/source/latex/kuvio/arrsy/Uarrsy.fd
texmf/source/latex/kuvio/arrsy/patchlevel_19
texmf/source/latex/kuvio/doc-src/README
texmf/source/latex/kuvio/doc-src/eg/eg01b.tex
texmf/source/latex/kuvio/doc-src/eg/eg02.tex
texmf/source/latex/kuvio/doc-src/eg/eg02A4.tex
texmf/source/latex/kuvio/doc-src/eg/eg03.tex
texmf/source/latex/kuvio/doc-src/eg/eg04.tex
texmf/source/latex/kuvio/doc-src/eg/eg05.tex
texmf/source/latex/kuvio/doc-src/eg/eg06a.tex
texmf/source/latex/kuvio/doc-src/eg/eg09.tex
texmf/source/latex/kuvio/doc-src/eg/eg12.tex
texmf/source/latex/kuvio/doc-src/eg/eg13.tex
texmf/source/latex/kuvio/doc-src/eg/eg15.tex
texmf/source/latex/kuvio/doc-src/eg/eg16.tex
texmf/source/latex/kuvio/doc-src/eg/eg17.tex
texmf/source/latex/kuvio/doc-src/eg/eg18.tex
texmf/source/latex/kuvio/doc-src/eg/eg19.tex
texmf/source/latex/kuvio/doc-src/eg/eg20.tex
texmf/source/latex/kuvio/doc-src/eg/eg20A4.tex
texmf/source/latex/kuvio/doc-src/eg/eg21.tex
texmf/source/latex/kuvio/doc-src/eps/face.eps
texmf/source/latex/kuvio/doc-src/eps/harebra.eps
texmf/source/latex/kuvio/doc-src/eps/plot.eps
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/auxfile.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/carrot.tex
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/cite.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/contents.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/counter.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/environ.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/equation.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/index.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/label.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/patchlevel_10
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/section.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/state.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/theorem.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/toc.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/basic/xr.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/misc/biblio.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/misc/rcs.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/sfss/fs/arrsy.fs
texmf/source/latex/kuvio/doc-src/macros/carrot/sfss/fs/bbm.fs
texmf/source/latex/kuvio/doc-src/macros/carrot/sfss/fs/bbold.fs
texmf/source/latex/kuvio/doc-src/macros/carrot/sfss/fs/cm.fs
texmf/source/latex/kuvio/doc-src/macros/carrot/sfss/fs/rsfs.fs
texmf/source/latex/kuvio/doc-src/macros/carrot/sfss/sfss.cd
texmf/source/latex/kuvio/doc-src/macros/carrot/sfss/sfss.df
texmf/source/latex/kuvio/doc-src/macros/carrot/sfss/sfss.fs
texmf/source/latex/kuvio/doc-src/macros/misc/calc.tex
texmf/source/latex/kuvio/doc-src/macros/misc/listing.tex
texmf/source/latex/kuvio/doc-src/macros/misc/verbatim.tex
texmf/source/latex/kuvio/doc-src/revision_2.5.12
texmf/source/latex/kuvio/doc-src/tdwk-A4.ccx
texmf/source/latex/kuvio/doc-src/tdwk-A4.cd
texmf/source/latex/kuvio/doc-src/tdwk-A4.cxr
texmf/source/latex/kuvio/doc-src/tdwk-A4.idx
texmf/source/latex/kuvio/doc-src/tdwk-A4.ind
texmf/source/latex/kuvio/doc-src/tdwk-A4.tex
texmf/source/latex/kuvio/doc-src/tdwk-A4.tmp
texmf/source/latex/kuvio/doc-src/tdwk-A4.toc
texmf/source/latex/kuvio/doc-src/tdwk-e.tex
texmf/source/latex/kuvio/doc-src/tdwk-r.tex
texmf/source/latex/kuvio/doc-src/tdwk-s.tex
texmf/source/latex/kuvio/doc-src/tdwk.cd
texmf/source/latex/kuvio/doc-src/tdwk.ist
texmf/source/latex/kuvio/doc-src/tdwk.tex
texmf/source/latex/kuvio/doc-src/tdwk/eg01b.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg01b.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg02A4.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg02A4.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg03.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg03.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg04.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg04.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg05.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg05.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg06a.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg06a.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg09.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg09.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg12.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg12.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg13.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg13.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg15.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg15.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg16.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg16.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg17.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg17.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg18.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg18.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg19.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg19.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg20A4.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg20A4.kuv
texmf/source/latex/kuvio/doc-src/tdwk/eg21.kdg
texmf/source/latex/kuvio/doc-src/tdwk/eg21.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-1.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-1.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-10.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-10.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-11.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-11.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-12.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-12.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-13.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-13.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-14.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-14.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-15.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-15.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-16.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-16.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-17.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-17.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-18.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-18.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-19.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-19.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-2.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-2.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-20.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-20.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-21.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-21.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-22.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-22.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-23.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-23.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-24.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-24.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-25.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-25.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-26.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-26.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-27.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-27.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-28.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-28.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-29.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-29.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-3.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-3.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-30.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-30.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-31.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-31.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-32.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-32.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-33.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-33.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-34.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-34.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-35.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-35.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-36.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-36.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-37.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-37.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-38.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-38.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-39.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-39.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-4.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-4.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-40.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-40.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-41.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-41.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-42.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-42.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-43.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-43.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-44.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-44.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-45.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-45.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-46.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-46.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-47.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-47.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-48.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-48.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-49.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-49.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-5.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-5.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-50.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-50.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-51.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-51.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-52.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-52.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-53.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-53.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-6.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-6.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-7.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-7.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-8.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-8.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-9.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-9.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-1.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-1.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-10.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-10.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-11.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-11.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-12.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-12.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-13.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-13.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-14.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-14.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-15.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-15.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-16.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-16.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-17.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-17.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-18.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-18.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-19.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-19.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-2.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-2.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-20.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-20.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-21.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-21.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-22.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-22.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-23.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-23.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-24.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-24.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-25.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-25.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-26.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-26.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-27.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-27.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-28.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-28.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-29.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-29.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-3.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-3.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-30.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-30.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-31.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-31.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-32.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-32.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-33.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-33.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-34.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-34.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-35.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-35.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-36.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-36.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-37.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-37.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-38.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-38.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-39.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-39.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-4.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-4.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-40.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-40.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-41.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-41.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-42.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-42.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-43.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-43.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-44.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-44.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-45.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-45.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-46.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-46.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-47.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-47.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-48.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-48.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-49.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-49.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-5.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-5.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-50.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-50.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-51.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-51.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-52.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-52.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-53.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-53.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-54.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-54.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-55.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-55.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-56.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-56.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-57.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-57.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-58.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-58.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-59.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-59.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-6.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-6.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-60.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-60.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-61.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-61.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-62.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-62.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-63.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-63.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-64.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-64.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-65.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-65.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-66.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-66.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-67.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-67.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-68.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-68.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-69.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-69.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-7.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-7.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-70.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-70.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-71.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-71.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-72.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-72.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-73.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-73.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-74.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-74.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-75.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-75.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-8.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-8.kuv
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-9.kdg
texmf/source/latex/kuvio/doc-src/tdwk/tdwk-s-9.kuv
texmf/source/latex/kuvio/patchlevel_216
    </TPM:SourceFiles>
    <TPM:Provides>package/kuvio</TPM:Provides>
  </rdf:Description>
</rdf:RDF>


==> xypic.tex <==
%% xypic.tex from $Id: xypic.doc,v 3.3 1996/12/19 03:31:56 krisrose Exp $
%%
%% Xy-pic v2 compatibility loading.
%% Copyright (c) 1993-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\input xyv2
\endinput

